GRASP: Graph Alignment through Spectral Signatures

What is the best way to match the nodes of two graphs? This graph alignment problem generalizes graph isomorphism and arises in applications from social network analysis to bioinformatics. Some solutions assume that auxiliary information on known matches or node or edge attributes is available, or utilize arbitrary graph features. Such methods fare poorly in the pure form of the problem, in which only graph structures are given. Other proposals translate the problem to one of aligning node embeddings, yet, by doing so, provide only a single-scale view of the graph. In this paper, we transfer the shape-analysis concept of functional maps from the continuous to the discrete case, and treat the graph alignment problem as a special case of the problem of finding a mapping between functions on graphs. We present GRASP, a method that first establishes a correspondence between functions derived from Laplacian matrix eigenvectors, which capture multiscale structural characteristics, and then exploits this correspondence to align nodes. Our experimental study, featuring noise levels higher than anything used in previous studies, shows that GRASP outperforms state-of-the-art methods for graph alignment across noise levels and graph types.

==> content/93.preliminaries-old.tex <==
%!TEX root=../main.tex
\section{Problem Setting}\label{sec:problem}

% moved here from introduction
\pk{{\spara{Graph Alignment.}} Consider two undirected graphs, $G_1 = (V_1, E_1)$ and $G_2 = (V_2, E_2)$, where $V_*$ are node sets. Without loss of generality we assume that $|V_1|=|V_2|=n$. $E_* \subseteq V_* \times V_*$ are edge sets and $A_1$ and $A_2$ are adjacency matrices.

\vspace{-1mm}
\begin{definition}\label{def:alignment}
Given two graphs $G_1=(V_1,E_1)$ and $G_2=(V_2,E_2)$, a graph alignment $R:V_1 \rightarrow V_2$ is an injective function that maps nodes of $G_1$ to nodes of $G_2$.
\end{definition}
\vspace{-1mm}

The graph alignment problem finds such an injective function, which, expressed as a permutation matrix $P$, minimizes the difference $\|PA_1P^\top-A_2\|^2$. In case of isomorphic graphs, there exists a $P$ such that $PA_1P^\top = A_2$, i.e., aligns the two graphs exactly. 
We are interested in the general, unrestricted problem case, in which there are no additional constraints on node attributes or matches known in advance. 
The problem is $\mathbf{NP}$-hard~\cite{cook71}; a popular way to address it is to match nodes among the two graphs guided by appropriate node representations. The challenge is then to (i) find such an appropriate node representation that captures graph structure at both local and large scale, going beyond mere node degree or ego-net structure, including neighborhood connectivity and community structure, and (ii) match nodes having similar characteristics on different levels, from their relationship to the whole graph over community membership to node degrees and neighborhoods. 
\dm{A graph representation that captures such properties is the eigenvectors and eigenvalues of the graph Laplacian~\cite{tsitsulin18kdd}.}}
% Mind that the graph's Laplacian is just an operator, not a representation -
% END of Page 2, 01dec2019

\dm{
\begin{table}[t!]
	\centering
	\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
	% \vspace{-.3cm}
% 	\def\arraystretch{1}
	\begin{tabularx}{\linewidth}{ R p{6.8cm} }
		\toprule
		\textbf{Symbol} & \textbf{Meaning} \\
		\midrule
		$\graph_*$ & Graph $\graph_* = (\nodes_*,\edges_*)$ with node set  $\nodes_*$, edge set  $\edges_*$ \\
		$A$ & Graph adjacency matrix, $A_{ij}{=}1$ if $(i,j){\in}\edges$, $0$ otherwise \\
		$\lapl$ & Graph Laplacian $\lapl{=}\eye-D^{-\frac{1}{2}}AD^{-\frac{1}{2}}$, $D_{ii}{=}\sum_{j=1}^n A_{ij}$\\
		$\Phi, \Psi$ & $\lapl_1$'s eigevenctor matrix $\Phi = [\phi_1 \phi_2 \ldots \phi_n]$, $\Psi$ equivalent for $\lapl_2$ \\
		$H_t^G$ & Heat kernel $H_t = \Phi e^{-t\Lambda}\Phi^\top$ for graph $G$\\
		$F, G$ & Corresponding functions $F{=}[f_1 f_2... f_q], f_i= \sum_{j=1}^n e^{-t_i\lambda_j}\phi_j\odot\phi_j$, $G$ is equivalent for graph $G_2$ \\
		$C$ & Corresponding matrix $F^\top\Phi=G^\top\Psi C$ \\
		$M$ & Base alignment matrix\\
		\bottomrule
	\end{tabularx}
	\caption{Table of the main symbols.}
	\label{tbl:notation}
	\vspace{-5mm}
\end{table}
}

\subsection{Graph Spectrum}

\pk{A graph's \emph{adjacency matrix} $A \in \{0,1\}^{n\times n}$ is a binary matrix where $A_{ij}=1$ if there is an edge between nodes $i$ and $j$ and $A_{ij}=0$ otherwise.
The \emph{degree matrix} $D$ of a graph is a diagonal matrix of node degrees, i.e., $D_{ii}=\sum_{j=1}^n A_{ij}$. The \emph{normalized graph Laplacian}, is the matrix $\lapl=\eye-D^{-\frac{1}{2}}AD^{-\frac{1}{2}}$, its spectral decomposition is $\lapl=\Phi\Lambda\Phi^\top$, where $\Lambda$ is a diagonal matrix of eigenvalues, $\{\lambda_1, \ldots, \lambda_n\}$, i.e., the graph's \emph{spectrum} that encodes structural information about communities, degree distribution, and diameter, and $\Phi$ is a matrix of eigenvectors, $\Phi = [\phi_1 \phi_2 \ldots \phi_n]$; eigenvectors form an orthogonal basis, hence we can express any vector $v\in \mathbb{R}^n$ as a linear combination $v=\sum_j^n a_j\phi_j$ with $a_j \in \mathbb{R}$.}

\input{figs/eifuns.tex}

\subsection{Functional Maps}\label{sec:maps}

\jh{
\pk{Consider two isomorphic graphs, $G_1$ and $G_2$, and a function $\tau: V_1 \rightarrow V_2$ that gives the ground truth mapping between nodes of $G_1$ and $G_2$. In addition, consider a function $f: V_1\rightarrow \mathbb{R}$ that maps nodes to real values, such as a node's degree or an indicator function $\delta_i$ yielding $1$ for a given node: 
\[\delta_i(v_j)=\begin{cases}
1 & \text{if } j=i\\
0& \text{else}  
\end{cases}\label{eq:delta}\]

If we compose $f$ and $\tau$ as \dm{$g=\tau^{-1}\circ f$ with $g: V_2\rightarrow \mathbb{R}$}, where $\tau^{-1}:V_2 \rightarrow V_1$ is the $\tau$'s inverse, we map~$f$ to graph $G_2$. Thus, the mapping function $\tau$ also implies a mapping of functions from $G_1$ to $G_2$. Assume we know $f$ and $g$, but not $\tau$; for example, $f(v_i)=deg(v_i)$ and $g(v'_i)=deg(v'_i)$. Given that $G_1$ and $G_2$ are isomorphic, if we set $\Phi$ and $\Psi$ as the eigenvectors of $\lapl_1$ and $\lapl_2$, respectively, then $f=\sum_{i=1}^n a_i \Phi_i$ and $g=\sum_{i=1}^n b_i \Psi_i$, where $a_i=\pm b_i$ \dm{as in isomorphic graphs eigenvectors \dm{correspond up to vector orientation, i.e $\phi_i=\tau\circ\psi_i$}}; we can thus find an \emph{orthogonal diagonal correspondence matrix} $C$ such that $a_i=c_{i,i}\cdot b_i$, i.e. \dm{$f^\top\Phi = g^\top\Psi C$}.}
%% why claim they exist since we set them as eigenvectors?
%there exist two orthogonal bases $\Phi$ and $\Psi$, such that.
%% this is not defined: how is \circ applied on \Phi and \si?
%where $\Phi_i=\Psi_i\circ t$ for $1\leq i\leq n$.
%We can guarantee the existence of such bases for isomorphic graphs, even without knowing~$t$.
%% do we set them this way, or assume their existence?
%If we set $\Phi$ and $\Psi$ as the eigenvectors of $\lapl_1$ and $\lapl_2$, then it holds that $\Phi_i=\Psi_i\circ t$, up to sign changes. We can now decompose $f$ and $g$ as
%Given that $\Phi$ and $\Psi$ hold up to sign changes, we know that $a_i=\pm b_i$ and can thus solve for $C$ in $\Phi=C\Psi$, such that $a_i=c_{i,i}\cdot b_i$.
%% we did not assume we did not know g; we assumed we did not know t!
%With all the made assumptions, we can use $C$ to map functions $f$ across graphs for which we do not know $g$. Considering Equation \ref{eq:delta}, we can obtain the coefficients using $C$ and with this reconstruct $\delta'$ on $G_2$, which then will peak for the corresponding node in $G_2$.
}

% \pk{Consider a function $f:V\rightarrow\mathbb{R}$, which maps nodes of a graph $G = (V,E)$ to real values, and let the set $L^2(V)=\{f:V\rightarrow\mathbb{R}\}$ denote the set of all such functions for graph $G$. To solve the graph alignment problem, we first find a \emph{functional mapping} $T:L^2(V_1)\rightarrow L^2(V_2)$, for graphs $G_1=(V_1,E_1)$ and $G_2=(V_2,E_2)$, and then apply it on an indicator function $\delta_i(\cdot)$ on graph nodes defined as:
% \[\delta_i(v_j)=\begin{cases}
% 1 & \text{if } j=i\\
% 0& \text{else}  
% \end{cases}\]
% Assuming that $v_i$ corresponds to a node $v'_k$ in graph $G_2$, we apply $\delta$ to nodes in $G_2$ as well, and map such function among graphs by a \emph{functional map} $T$:

% \[T\circ \delta_i(v_j)=\begin{cases}
% 1 & \text{if } j=k\\
% 0& \text{else}  
% \end{cases}\]}  

\pk{This correspondence matrix $C$ effectively maps function coefficients from $G_1$ to $G_2$, even without knowing the ground truth mapping $\tau$. Our method obtains a correspondence matrix $C$ for one eigenvector-based function and applies that $C$ to the task of mapping the indicator function $\delta$ on $G_1$ to that on $G_2$, so as to constructs a node alignment. In Section~\ref{sec:solution}, we expand this idea to non-isomorphic graphs.}

% obsolete (same point in other words)
%\pk{We will determine $T$ indirectly in the following manner. First, we formulate a generic toolbox that determines the coefficients of a node-to-value function $f$ as a linear combination of a graphs' Laplacian eigenvectors. We use one case of such function to calculate a correspondence matrix $C$ that links such function coefficients among two graphs, and apply the same $C$ to the task of node alignment.}



\subsection{Heat Kernel}

\pk{To build and obtain a correspondence between structure-aware node-evaluated functions, we work with the \emph{heat kernel}, which was also used for similar purposes in~\cite{tsitsulin18kdd}:

\vspace{-1mm}
\begin{equation}
H_t = \Phi e^{-t\Lambda}\Phi^\top = \sum_{j=1}^n e^{-t\lambda_j}\phi_j\phi_j^\top
\end{equation}
\label{eq:heat-kernel}
\vspace{-1mm}

where $H_{t[ij]}$ measures the flow of heat from node $i$ to node $j$ at time $t$, as it diffuses from a node's neighborhood to the whole graph. 
We build our model functions over a sequence of time steps $t$ using the \emph{diagonal} of the heat kernel, which measures the heat flowing back to each node at time $t$. 

\dm{\spara{Multiscale property.} The value in the diagonal can be thought as the likelihood a node is reached in a diffusion process in time $t$. In the beginning of the diffusion, when $t < 1$, Equation~\ref{eq:heat-kernel} emphasises large $\lambda$, which corresponds to \emph{local} edge and ego-nets properties. On the other hand, as long as time passes, Equation~\ref{eq:heat-kernel} assigns larger values to smaller eigenvalues, corresponding to \emph{global} properties, such as communities. We recall that $\phi_2$ is the Fiedler vector used to detect communities in spectral clustering.}
}

==> content/94.solution-old.tex <==
%!TEX root=../main.tex
\section{Solution}\label{sec:solution}

%\pk{We outline our solution.}
%\subsection{Corresponding Functions}

% Story 1 

% - Let us start our discussion with assuming that we are given a bijective mapping between the nodes of the graph
% - If we had such function we could apply the indicator function on nodes of graph G_2 to obtain nodes on the graph G_2
% - This reasoning work on any real valued function f,g on nodes in G_1, G_2. b7y8
% - That means that if we know a set of functions which corresponds one to another we could recover the behavior of the indicator functions on the nodes.
% - However, there are two problems: not all functions can act as good corresponding functions, and not all represent the behaviour of the indicator function. 
% - Can we say here that Heat is a good choice as the indicator function can be immediately represented as H_{0,i}? 
% - So if we are able to align functions on G_1 and G_2 we will be able to align nodes in the two graphs by means of representations over the nodes (Good!)
% Now how do we find C? 
% What happens if graphs are not close to be isomorphic? Base alignment











\pk{
We build our solution around \emph{corresponding functions} $f_i$ expressed as linear combinations of the graph's Laplacian orthogonal eigenvectors $\phi_1,\ldots,\phi_n$, i.e., $f_i = \sum_{j=1}^n a_j\phi_j$. 
Let $F \in \reals^{n\times q}, F = [f_1, \ldots, f_q]$ be the matrix containing the diagonals of the heat kernel of $G_1$, $H_t^{G_1}$, over $q$ time steps\footnote{In our experiments we select $q=100$ values evenly spaced on the linear scale in the range [0.1, 50].} as vectors, i.e., ${f_i= \sum_{j=1}^n e^{-{t_i}\lambda_j}\phi_j \odot \phi_j}$, where $\odot$ denotes the element-wise vector product. Likewise, the matrix $G \in \reals^{n\times q}, G = [g_1, \ldots, g_q]$ contains the diagonals of $H_t^{G_2}$, the heat kernel of $G_2$. 
While the $q$ \emph{columns} of $F$ and $G$ contain the same time-dependent heat-kernel-diagonal functions evaluated on the nodes of two different graphs, their $n$ \emph{rows} (i.e., nodes) are not aligned. We need to obtain such a node alignment.}

\subsection{Correspondence Matrix}

\pk{We approximate each function $f_i$ using only the first $k$ eigenvectors, as done, by analogy, with eigenvectors of the Laplace-Beltrami operator on shapes~\cite{belkin06},
%for Fourier series expansion in the manner of a low-pass filter~\cmt{REF}. % is this needed here?
and thereby calculate the corresponding function matrices $F$ and $G$.} 
\dm{$F$ and $G$ can be thought as coefficient matrices of the linear combination $F^\top\Phi$ and $G^\top\Psi$ of the eigenvectors of $G_1$ and $G_2$ Laplacians, respectively. 
With a slight abuse of notation, we denote with $\Phi$ and $\Psi$ the first $k$ eigenvectors. 
In the projection of the functions on the first $k$ eigenvectors, we would like the corresponding functions to be equal up to a coefficient matrix $C \in \reals^{k \times k}$. 
In the particular case of isomorphic graphs $F^\top\Phi=G^\top\Psi C$ and $C$ is diagonal.
% therefore, every function $f_i$ is composed as $\Phi f_i = C $
% From these \emph{coefficient matrices} \dm{$A,B \in \reals^{k\times q}$}, such that  $f_i = \sum_{j=1}^k A_{ij}\phi_j$ and $g_i = \sum_{j=1}^k B_{ij}\jh{\psi}_j$ can be calculated, from which we aim to derive the correspondence matrix $C \in \reals^{k\times k}$ as $B=CA$. 
Instead of solving for $C$ here, we exploit the fact that $C$ is diagonal and use an approach similar to~\cite{kovnatsky13coupled}, 
Therefore, we solve $k{\cdot}q$ equations with $k$ variables defined as:}


\begin{equation}
    \begin{bmatrix}
    \diag(g_1^\top\Psi)\\
    \vdots\\
    \diag(g_q^\top\Psi)
\end{bmatrix}
    \begin{bmatrix}
    c_{11}\\
    \vdots\\
    c_{kk}
\end{bmatrix}
=    \begin{bmatrix}
    \Phi^\top f_1\\
    \vdots\\
    \Phi^\top f_q
\end{bmatrix}
\label{eq:corrmat}
\end{equation}

\dm{The solution to the above can be obtained by minimizing the L2-difference $\|\cdot\|^2_2$ among the left and right side of Eq.~\ref{eq:corrmat}.}

% \jh{With this matrix $C$, we can now map an arbitrary new function $f':V_1\rightarrow\reals$ from $G_1$ to its unknown counterpart $g':V_2\rightarrow\reals$ on $G_2$ by (1) decomposing $f'$ into coefficients $a'_1,\ldots, a'_k$ (2) transforming these coefficients into the coefficients $b'_1,\ldots b'_k$ with $b'_i=c_{ii}a'_i$ and (3) obtaining $g'$ as $\sum_{i=1}^k b'_i\Psi_i$.

% Until now, we have made one key assumption: We assumed that $\Phi$ and $\Psi$ perfectly correspond, i.e. $\phi_i=\pm \tau^{-1}\circ\psi_i$. This only holds for isomorphic graphs.
% }
%We then derive \emph{coefficient matrices} \dm{$A,B \in \reals^{k\times q}$}, such that  $f_i = \sum_{j=1}^k A_{ij}\phi_j$ and $g_i = \sum_{j=1}^k B_{ij}\jh{\psi}_j$, \dm{and calculate \emph{a diagonal matrix} $C^{k\times k}$ that solves

%\begin{equation}\label{eq:correspondence}
%    \argmin_{C\in\reals^{k\times k}} \|C A - B\|^2
%\end{equation}

%The solution to the optimization in Equation~\ref{eq:correspondence} is obtained by least squares fitting applied for each element of $C$.}}



\subsection{Base Alignment}
\label{ssec:basealign}


% DM: Don't need to say this. 
%\jh{For this Section, we draw on an approach proposed in~\cite{Kovnatsky13}, which solved an equivalent problem for shapes.} 
\pk{We have hitherto assumed that the graphs to be aligned, $G_1$ and $G_2$, are isomorphic, hence their eigenvectors correspond to each other with possible sign changes and an orthogonal and diagonal correspondence matrix $C$ exists. 
However, if the graphs are not isomorphic, then their eigenvectors diverge and a diagonal matrix $C$, which we enforce, cannot capture their relationship well. \dm{Figure~\ref{fig:spectra} highlights this issue: at a high level the eigenvectors underline common structures, but they differ at the node level.} In this case, we need to \emph{align} the two eigenvector bases before we consider aligning corresponding vectors and, eventually, nodes. 
We express this \dm{\emph{base alignment}~\cite{kovnatsky13coupled}} in terms of \dm{an alignment matrix $M$.}
% does rotation fully express base alignment? if so, the above is OK.
%\red{coupling? matrices $F$ and $G$? Provide all missing definitions}.

%\spara{Goal.} eigenvector matrices that are both diagonalizing the graph laplacian (because then they are still approx eigenvectors and have this nice 1 to k property \re{[which property is that? define it.]}) and are coupled (because then they are similar across graphs)

\dm{\spara{Alignment matrix.} We align the eigenvectors $\Psi$ by a rotation matrix $M$ so as transform $\Psi$ into $\Phi$: $\hat{\Psi} = \Psi M$. Since $\lapl\Psi = \Psi\Lambda$, finding $\Psi$ is equivalent to the solution of following quadratic minimization problem which penalizes elements outside of the diagonal:
\[\min_{\Psi} \off(\Psi^\top \lapl_2\Psi)~\text{s.t.}~\Psi^\top\Psi=\eye\]

\noindent where $\off(\cdot)$ denotes the sum of squared off-diagonal elements. 
Moreover, since the eigenvectors are orthonormal, $\Psi^\top\Psi=I$ and for $G_2$'s graph Laplacian eigenvectors $\Lambda_2$, $\Psi^\top \lapl_2\Psi = \Psi^\top \Psi\Lambda_2 = \Lambda_2$, and $M^\top \Psi^\top\lapl_2\Psi M=M^\top\Lambda_2 M$. 
%Here $\Lambda_2$ refers to the eigenvalues of $\lapl_2$. 
Putting the above together, our diagonalizing term is:

\[\min_{M} \off(M^\top \Lambda_2M)~\text{s.t.}~M^\top M=I\]

As we are minimizing over orthogonal matrices we can equivalently express the objective above as a minimization over orthogonal matrices of size $n \times n$ $S(n,n)$:

\[\min_{M\in S(n,n)}\off(M^\top\Lambda_2 M)\]

\spara{Coupling.} The correspondence $\tau: G_1\rightarrow G_2$ so that $\phi_i\approx\tau\circ\psi$ translates to 

\[\min_\Phi\|F^\top\Phi-G^\top\Psi M\|_F^2\]

\noindent where $F$ and $G$ contain each graphs's corresponding functions.
% repetition
%Combining that with the rotation matrix $B$, we get:
%\[\min_{B\in S(k,k)}\mu||F^\top\Phi-G\Psi B||_F^2\]
We combine the minimization terms for diagonalization and coupling to get the following minimization problem, with regularization factor~$\mu$ \dm{\footnote{$\mu =0.132$ in our experiments}}:

\begin{equation}
\min_{M\in S(n,n)}\off(M^\top\Lambda_2 M)+\mu\|F^\top\Phi-G^\top\Psi M\|_F^2
\label{eq:basealign}
\end{equation}

Given that the eigenvectors of isomorphic graphs match each other with sign changes, we initialize $M$ as a diagonal matrix with:

\[b_{i,i}=
\begin{cases}
+1 & \text{if }~  \|F^\top\phi_i-G^\top\psi_i\|\leq\|F^\top\phi_i+G^\top\psi_i\|\\
-1 & \text{otherwise}  
\end{cases}
\]
}}

% \red{What method is used to solve this? What about the text commented out here?}
\dm{Equation~\ref{eq:basealign} leads to a smooth optimization problem which can be solved with trust-region methods on Riemannian manifolds~\cite{absil2007trust}.}
% as implemented in pymanopt. }

\dm{\spara{Scalability.} In order to avoid computing all eigenvectors $n\times n$, we exploit the fact that we only need the first $k$ eigenvectors for calculating $C$. So we only align the first $k$ eigenvectors of $\Psi$ to the first $k$ eigenvectors of $\Phi$, i.e $\bar{\Phi}=\hat{\Psi} =\bar{\Psi} M$ with $\bar{\Phi}=[\phi_1,\ldots,\phi_k]$ and $\bar{\Psi}=[\psi_1,\ldots,\psi_k]$. The optimization problem in Equation \ref{eq:basealign} then becomes

\begin{equation}
\min_{M\in S(k,k)}\off(M^\top\bar{\Lambda}_2 M)+\mu\|F^\top\bar{\Phi}-G^\top\bar{\Psi} M\|_F^2
\end{equation}
with $\bar{\Lambda}_2=\diag(\lambda_1,\ldots,\lambda_k)$.



After obtaining $M$, we use the eigenvectors in $\bar{\Phi}$ and the aligned eigenvectors $\hat{\Psi} =\bar{\Psi}M$ in the next step for the final alignment of nodes.}
% \red{What method is used to solve this? What about the text commented out here?}
% We use a trust region method on Riemannian manifolds~\cite{absil2007trust} for solving Equation~\ref{eq:basealign}.



\subsection{Node-to-node correspondence}
\label{ssec:matching}
\dm{
% \begin{itemize}
%     \item Look for functions with same coefficients
%     \item Easy function: delta functions $\rightarrow$ what are their coefficients
%     \item heat kernel row at time $t=0$
%     \item imagine as matching of node descriptors
% \end{itemize}

In order to compute the node-to-node correspondence for graph alignment, we exploit the fact that in the ideal case \emph{corresponding functions have the same coefficients.} We consider the delta function $\delta_i(\cdot)$ introduced in Section~\ref{sec:maps} as corresponding function; these functions yield a $n\times n$ identity matrix. The idea now is to match the coefficient vectors of these corresponding indicator functions, as for two matching nodes $v_i\in V_1$ and $v'_j\in V2$, the coefficients of $\delta_i$ and $\delta_j$ for $\bar{\Phi}$ and $\hat{\Psi}$ should be the same. 

We express such functions as vectors of coefficients starting out from the fact that the vector of $\delta_i$ is the $i$th row of the heat kernel at $t=0$:

\vspace{-2mm}
\[\delta_i=H_{i,t=0}^{G_1}=\sum_{j=1}^n \phi_{ij}\phi_j\]
\vspace{-1mm}

The computation for delta functions on $G_2$ follows equivalently using $\hat{\Psi}$ instead of $\bar{\Phi}$. It follows that the coefficients expressing $\delta_i$ as a linear combination of the first $k$ eigenvectors are $\Phi_{i1}, \ldots, \Phi_{ik}$. 
We thus can set $\bar{\Phi}^\top$ and $C\hat{\Psi}^\top$ as coefficient matrices of the delta functions, aligned by $C$. Rows correspond to the first $k$ Laplacian eigenvectors, while now columns stand for graph nodes. 
Finally, we need to assign matching coefficient vectors, i.e. columns of $\bar{\Phi}^\top$ and $C\hat{\Psi}^\top$ to each other. This can be seen as matching node descriptors of corresponding nodes. 
The problem turns into a \emph{linear assignment problem}, where we use a linear assignment algorithm such as \textbf{nearest neighbor search} or \textbf{Jonker-Volgenant (JV)~\cite{jonker1987shortest}} to obtain an one-to-one matching between the columns of $\bar{\Phi}^\top$ and those of $C\hat{\Psi}^\top$, and hence an alignment of nodes in $G_1$ and $G_2$.
}


% then we use a \emph{linear assignment algorithm} such as \textbf{nearest neighbor search} or \textbf{Jonker-Volgenant (JV)~\cite{jonker1987shortest}} to obtain an one-to-one matching between the columns of $C F^\delta$ and those of $G^\delta$ \cmt{what objective function is minimized here?}, and hence an alignment of nodes in $G_1$ to nodes in $G_2$.}
\dm{This vindicates the \emph{flexibility} of \thiswork, which can supply different matching algorithms and different transformations on the coefficient matrix, without changing the overall framework. 
Section~\ref{ssec:variants} compare variants using nearest neighbor or JV.}
%SortGreedy~\cite{doka2015k}



\input{figs/alg-grasp.tex}



\section{Our algorithm: \thiswork}
\dm{Putting all together, our \thiswork depicted in Algorithm~\ref{alg:grasp} consists of six steps.

\spara{Compute eigenvectors.} In the first step, calculate the Laplacians $\lapl_1,\lapl_2$ of the two graphs $G_1$ and $G_2$. Then compute the eigenvectors $\Phi,\Psi$ and eigenvalues $\Lambda_1,\Lambda_2$ by the eigendecomposition $\lapl_1=\Phi\Lambda_1\Phi^\top$ and $\lapl_2=\Psi\Lambda_2\Psi^\top$.

\spara{Compute corresponding functions.}
In the second step, calculate the matrices of corresponding functions $F=[f_1,\ldots,f_q]$ and $G=[g_1,\ldots,g_q]$ as diagonals of the heat kernel at time steps $[t_1,\ldots,t_q]$ with $f_i= \sum_{j=1}^n e^{-{t_i}\lambda_j}\phi_j \odot \phi_j$ and $g_i$ equivalently using $\Psi$.


\spara{Base alignment.}
After  the corresponding functions are calculated, obtain the base alignment matrix $M$ by minimizing equation \ref{eq:basealign}. Then align the first $k$ columns of $\Psi$, denoted by $\bar{\Psi}$ to the corresponding first $k$ columns $\bar{\Phi}$ of $\Phi$ as $\hat{\Psi}=\bar{\Psi}M$.

\spara{Calculate correspondence matrix.}
Under the assumption that $C$ is a diagonal matrix, calculate its diagonal elements $c_{11},\ldots,c_{kk}$ by minimizing the following least squares problem:
\begin{equation*}
\min_{[c_{11},\ldots,c_{kk}]^\top}\left\Vert\begin{bmatrix}
    \diag(g_1^\top\bar{\Psi})\\
    \vdots\\
    \diag(g_q^\top\bar{\Psi})
\end{bmatrix}
    \begin{bmatrix}
    c_{11}\\
    \vdots\\
    c_{kk}
\end{bmatrix}
-  \begin{bmatrix}
    \hat{\Phi}^\top f_1\\
    \vdots\\
    \hat{\Phi}^\top f_q
\end{bmatrix}
\right\Vert_2^2
\end{equation*}
We then set $C=diag(c_{11},\ldots,c_{kk})$.

\spara{Node alignment.} Using the fact that corresponding functions should have the same coefficients on both graphs, obtain the coefficients of the indicator functions for all nodes as  $\bar{\Phi}^\top$ and $C\hat{\Psi}^\top$. In order to get the final alignment of nodes, align the columns of $\bar{\Phi}^\top$ and $C\hat{\Psi}^\top$ with a linear assignment algorithm.
}
%Solve for node-to-node correspondence~\cite{DBLP:journals/tog/OvsjanikovBSBG12} 
 %   \begin{itemize}
       % \item New set of corresponding functions: delta functions which are peaked at the node itself, so $n$ corresponding functions
        %\item Delta function for node $i$ can be expressed as heat kernel row at time $t=0$: $ H_t=\sum_{j=1}^n \phi_j\phi_j^\top  $
       % \item coefficients of $\delta_i$: $\Phi_{i,1},\ldots\Phi_{k,i}$ 
        %\item Coefficient matrix: columns are points, rows are eigenvector
 %       \item Matching: nearest neighbor search/ sortgreedy \cite{doka2015k}/ Jonker-Volgenant \cite{jonker1987shortest} (some linear assignment solver similar to hungarian)  matching on the columns of $C\Phi^{G_1}$ and $\Phi^{G_2}$
%    \end{itemize}

% \subsection{Iterative Closest Point}

% \pk{The matrix $C$ we obtain would ideally render each column in  $C F^\delta$ identical to some column in $G^\delta$, and vice versa. As this will not be the case, we refine the initial $C$ iteratively by the \emph{iterative closest point} method~\cite{besl1992method}: in each step, we set it as $\arg\min_C \sum||Cn_1-n_2||$, where $n_1$ and $n_2$ are pairs of columns in $C F^\delta$ and $G^\delta$ that match best.}
    % Challenges when applying shape matching approach to data/graph mining:
    % \begin{itemize}
    %     \item Eigenvectors of different sizes for graphs with different numbers of nodes $\rightarrow$ zero padding?
    %     \item On shapes, matching quality depends heavily on corresponding functions. For shapes, descriptors are used, which are comparably easy to obtain. How do we get something like this on graphs?
    %     \item Edge density/connectivity in sampled shapes is mostly similar. In graphs not. 
    %     \item If we have a pattern to match, is it better to match it to a similar pattern of higher or of lower density?
    % \end{itemize}
    
%    Random stuff:
%    \begin{itemize}
%        \item ''While experimentally it is known that often low-frequency harmonics have similar behavior (finding pro-trusions in shapes, a fact often employed for shape segmentation) \cite{DBLP:journals/ijcv/Reuter10})'' (from \cite{DBLP:journals/cgf/KovnatskyBBGK13})$\rightarrow$ initialization of graph matching via part segmentation using this
%        \item Iterative Refinement
%        \item Find nodes with similar characteristics
%   \item Features = curves with walk (Interactive Curve Constrained Functional Maps)
%    \item Use information from the spectrum as constraints for the matching process
%    \item Find corresponding nodes via degree similarity \cite{DBLP:conf/cikm/HeimannSSK18}
%    \item Constraints on nodes which totally cannot match
%    \end{itemize}

==> figs/exp_accuracy.tex <==
\begin{figure*}
\centering
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/arenas_accs_hun.png}  
  \caption{Arenas}
  \label{fig:quality:others_arenas}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/facebook_accs_hun.png} 
  \caption{Facebook}
  \label{fig:quality:others_facebook}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/CA-AstroPh_accs_hun.png} 
  \caption{CA-AstroPh}
  \label{fig:quality:others_CA-AstroPh}
\end{subfigure}
\vspace{-3mm}
\caption{Accuracy compared to REGAL~\protect\cite{heimann18regal} and Low Rank EigenAlign~\protect\cite{nassar2018lowrank}}
\label{fig:quality}
\vspace{-3mm}
\end{figure*}


% \begin{figure*}
% \centering
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figs/time_precomputed.png}  
%   \caption{Precomputed}
%   \label{fig:others_arenas}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figs/time_precomputed.png} 
%   \caption{Not precomputed}
%   \label{fig:others_facebook}
% \end{subfigure}
% \vspace{-3mm}
% \caption{Computation times of GASP and its closest competitor REGAL}\label{fig:time}
% \vspace{-3mm}
% \end{figure*}

==> figs/exp_basealign.tex <==
% \begin{figure*}
% \centering
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figs/arenas_others_accs_nn_hun.png}  
%   \caption{Arenas}
%   \label{fig:others_arenas}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figs/facebook_others_accs_nn_hun.png} 
%   \caption{Facebook}
%   \label{fig:others_facebook}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figs/CA-AstroPh_others_accs_nn_hun.png} 
%   \caption{CA-AstroPh}
%   \label{fig:others_CA-AstroPh}
% \end{subfigure}
% \vspace{-3mm}
% \caption{Accuracy compared to REGAL~\protect\cite{heimann18regal} with nearest neighbor alignment and jv alignment}\label{fig:parameters}
% \vspace{-3mm}
% \end{figure*}


\begin{figure*}
\centering
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/variants_arenas.png}  
  \caption{Arenas}
  \label{fig:variants:others_arenas}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/variants_facebook.png} 
  \caption{Facebook}
  \label{fig:variants:others_facebook}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/variants_CA-AstroPh.png} 
  \caption{CA-AstroPh}
  \label{fig:variants:others_CA-AstroPh}
\end{subfigure}
\vspace{-3mm}
\caption{Accuracy with and without aligning bases, with nearest neighbor and jv}
\label{fig:variants}
\vspace{-3mm}
\end{figure*}


==> figs/exp_tuning.tex <==
\begin{figure*}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/arenas_k.png}  
  \caption{Arenas, $q=100$}
  \label{fig:arenas_k}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/facebook_k.png} 
  \caption{Facebook, $q=100$}
  \label{fig:facebook_k}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/arenas_q.png}  
  \caption{Arenas, $k=20$}
  \label{fig:arenas_q}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/facebook_q.png} 
  \caption{Facebook, $k=20$}
  \label{fig:Facebook_q}
\end{subfigure}
\vspace{-3mm}
\caption{Accuracy on the facebook and arenas graphs for different numbers of corresponding functions $q$ and different numbers of eigenvectors $k$ for noise levels 5\%, 10\% and 15\%.}
\label{fig:parameters}
\vspace{-3mm}
\end{figure*}

% \begin{figure*}
% \centering
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figs/variants_arenas.png}  
%   \caption{Arenas}
%   \label{fig:var_arenas}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figs/variants_facebook.png} 
%   \caption{Facebook}
%   \label{fig:var_facebook}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figs/variants_bingham.png}  
%   \caption{Bingham82}
%   \label{fig:var_CA-HepTh}
% \end{subfigure}
% \vspace{-3mm}
% \caption{Accuracy per graph for different noise levels for the different variants of our method.}
% \label{fig:gasp_variants}
% \vspace{-3mm}
% \end{figure*}

==> tables/tbl-notation.tex <==
% \dm{
\begin{table}[t!h]
	\centering
	\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
	%\vspace{-.3cm}
    %\def\arraystretch{1}
	\begin{tabularx}{\linewidth}{ R p{6.8cm} }
		\toprule
		\textbf{Symbol} & \textbf{Meaning} \\
		\midrule
		$\graph_*$ & Graph $\graph_* = (\nodes_*,\edges_*)$, nodes $\nodes_*$, edges  $\edges_*$ \\
		$A$ & Adjacency matrix, $A_{ij}{=}1$ if $(i,j){\in}\edges$ \\
		$\lapl$ & Laplacian $\lapl{=}\eye-D^{-\frac{1}{2}}AD^{-\frac{1}{2}}$, $D_{ii}{=}\sum_{j=1}^n A_{ij}$\\
		$\Phi, \Psi$ & $\lapl_1$ and $\lapl_2$  eigevenctor matrices\\ %$\Phi = [\phi_1 \phi_2 \ldots \phi_n]$\\
		$H_t^\Gr$ & Heat kernel $H_t = \Phi e^{-t\Lambda}\Phi^\top$ for graph $\Gr$\\
		$F, G$ & $\Gr_1, \Gr_2$ corresponding functions \\%$F{=}[f_1 f_2 ... f_q], f_i= \sum_{j=1}^n e^{-t_i\lambda_j}\phi_j\odot\phi_j$ \\
		$C$ & Mapping matrix $F^\top\Phi=\Gr^\top\Psi C$ \\
		$M$ & Base alignment matrix\\
		\bottomrule
	\end{tabularx}
	\caption{Table of the main symbols.}\label{tbl:notation}
	\vspace{-8mm}
\end{table}
% }

==> tables/unready_tables.tex <==
\begin{table}
\caption{Elements we identified for graph matching (Embedding, similarity computation and matching) approaches and their correspondence in LRNetAlign, REGAL and our approach.}
\begin{center}
  \begin{tabular}{| l || l | p{3cm} | l|}
    \hline
    & LREA & REGAL & Ours\\ \hline\hline
    Embedding &  & Descriptors calculated from egonet descriptor similarities & Spect. sigs \\ \hline
    Similarity &  & Compare sigs & Compare sigs\\ \hline
    Matching &  & NN matching & Hung. matching \\\hline
  \end{tabular}
  \label{tab:elements}
\end{center}
\end{table}

\begin{table}  
\caption{Given the graph alignment elements from Table \ref{tab:elements}, we can interchange these elements between REGAL and our approach.}
\begin{center}
  \begin{tabular}{| l | l | l | l |}
    \hline
      & Algorithm & Signature & Align\\ \hline
     & 0 & 0 & 0\\ \hline
     & 0 & 0 & 1\\ \hline
    REGAL & 0 & 1 & 0\\ \hline
    REGAL + H & 0 & 1 & 1\\ \hline
    Ours  & 1 & 0 & 0\\ \hline
    Ours + H & 1 & 0 & 1\\ \hline
     & 1 & 1 & 0\\ \hline
     & 1 & 1 & 1\\ \hline
  \end{tabular}
 \label{tab:combos}
\end{center}
\end{table}
